Auditing AI models for Verified Deployment under Semantic Specifications

Auditing trained deep learning (DL) models prior to deployment is vital for preventing unintended consequences. One of the biggest challenges in auditing is the lack of human-interpretable specifications for the DL models that are directly useful to the auditor. We address this challenge through a sequence of semantically-aligned unit tests, where each unit test verifies whether a predefined specification (e.g., accuracy over 95%) is satisfied with respect to controlled and semantically aligned variations in the input space (e.g., in face recognition, the angle relative to the camera). We enable such unit tests through variations in a semantically-interpretable latent space of a generative model. Further, we conduct certified training for the DL model through a shared latent space representation with the generative model. With evaluations on four different datasets, covering images of chest X-rays, human faces, ImageNet classes, and towers, we show how AuditAI allows us to obtain controlled variations for certified training. Thus, our framework, AuditAI, bridges the gap between semantically-aligned formal verification and scalability. A blog post accompanying the paper is at this link https://developer.nvidia.com/blog/nvidia-research-auditing-ai-models-for-verified-deployment-under-semantic-specifications

==> 0-packages.tex <==
% basic
\usepackage{color}
\usepackage{epsfig}
\usepackage{graphicx}
%\usepackage{ulem}

% figure and table
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{subcaption} % issues a warning with CVPR/ICCV format

% font and character
\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}

% layout
\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}

% ref
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,citecolor=gray]{hyperref}

% misc
\usepackage{algorithm, algorithmic}
\usepackage{enumerate}
% \usepackage[draft]{todonotes} % conflict with CVPR/ICCV/CORL format

\usepackage{titlesec}
\usepackage{verbatim} 


==> 2-related-works.tex <==
\section{Related Works}

\noindent\textbf{Adversarial robustness.} Multiple prior works have studied a subset of the audit problem in terms of adversarial robustness~\citep{adversarial1,adversarial2,IBP,zhang2018crown,Singh2019robustness,weng2018towards,singh2018fast,wang2018efficient,raghunathan2018certified,raghunathan2018semidefinite,dvijothamefficient2019}. Adversarial examples are small perturbations to the input (for images at the level of pixels; for text at the level of words) which mislead the deep learning model.
% to incorrectly predict the corresponding output. 
Generating adversarial examples has been widely studied~\citep{generateadversarial,athalye2018obfuscated,carlini2017adversarial,carlini2017towards,goodfellow2014explaining,madry2018towards,papernot2016distillation,xiao2019meshadv,xiao2018generating,xiao2018spatially,eykholt2018robust, chen2018attacking,xu2018structured,zhang2019limitations} and recent approaches have devised defenses against adversarial examples~\citep{guo2017countering, song2017pixeldefend, buckman2018thermometer, ma2018characterizing, samangouei2018defense,xiao2018characterizing,xiao2019advit,robustness,robustness1,IBP, crownIBP}. Some of these approaches like~\citep{IBP} and~\citep{crownIBP} provide provable verification bounds on an output specification based on the magnitude of perturbations in the input. These approaches have largely showed robustness and verification to norm bounded adversarial perturbations without trying to verify with respect to more semantically meaningful properties of the input. 

\noindent\textbf{Neural network interpretability.} With the rapid rise of highly reliable generative models, many recent works have sought to analyze the latent space of such models and how the latent space can be manipulated to obtain semantic variations in the output image.~\citep{paintbyword} use text embeddings from CLIP~\citep{CLIP} to perform directed semantic changes in the generated images, for example introduction of a particular artifact in the room or change in the color of a bird.~\citep{manipulation1,manipulation2,manipulation3} identify latent code dimensions corresponding to pose of the body/face, expression of the face, orientation of beds/cars in the latent space of generative models like PGGAN~\citep{PGGAN} and StyleGAN~\citep{stylegan}. By manipulating these latent dimensions, the output images can be controllably varied. In addition, there have been other papers that sought to understand what the neural network weights are learning in the first place~\citep{understanding1,beenkim} in an attempt to explain the predictions of the networks. 


% \noindent\textbf{Machine Learning with constraints.}

% \noindent\textbf{Verification of neural networks.} 

% \noindent\textbf{Bias, fairness, ethics.}

